Multi-Level Contrastive Learning for Dense Prediction Task

In this work, we present Multi-Level Contrastive Learning for Dense Prediction Task (MCL), an efficient self-supervised method for learning region-level feature representation for dense prediction tasks. Our method is motivated by the three key factors in detection: localization, scale consistency and recognition. To explicitly encode absolute position and scale information, we propose a novel pretext task that assembles multi-scale images in a montage manner to mimic multi-object scenarios. Unlike the existing image-level self-supervised methods, our method constructs a multi-level contrastive loss that considers each sub-region of the montage image as a singleton. Our method enables the neural network to learn regional semantic representations for translation and scale consistency while reducing pre-training epochs to the same as supervised pre-training. Extensive experiments demonstrate that MCL consistently outperforms the recent state-of-the-art methods on various datasets with significant margins. In particular, MCL obtains 42.5 AP$^\mathrm{bb}$ and 38.3 AP$^\mathrm{mk}$ on COCO with the 1x schedule fintuning, when using Mask R-CNN with R50-FPN backbone pre-trained with 100 epochs. In comparison to MoCo, our method surpasses their performance by 4.0 AP$^\mathrm{bb}$ and 3.1 AP$^\mathrm{mk}$. Furthermore, we explore the alignment between pretext task and downstream tasks. We extend our pretext task to supervised pre-training, which achieves a similar performance to self-supervised learning. This result demonstrates the importance of the alignment between pretext task and downstream tasks, indicating the potential for wider applicability of our method beyond self-supervised settings.

==> tables/citykey.tex <==
\begin{table*}[t]
\vspace{-0pt}
 \centering
\resizebox{0.8\linewidth}{!}{%
  \begin{tabular}{l|llllll|lll}
  \toprule
  \multirow{2}{*}{Methods} & \multicolumn{6}{c|}{Keypoint} & \multicolumn{3}{c}{Cityscapes} \\
    & AP$^\text{bb}$ & AP$_\text{50}^\text{bb}$  & AP$_\text{75}^\text{bb}$ & AP$^\text{kp}$  & AP$_\text{50}^\text{kp}$  & AP$_\text{75}^\text{kp}$  &  mIoU & AP$^\text{mk}$  & AP$_\text{50}^\text{mk}$ \\
  \midrule
  Supervised & 57.5 & 84.0 & 63.0 & 65.6 & 87.0 & 71.3 & 72.9 & 31.8 & 58.5  \\
  SoCo~\cite{wei2021aligning} & 58.0\gly{+0.5} & 84.3\gly{+0.3} & 64.2\gly{+1.2} & 65.9\gly{+0.3} & 87.0\gly{+0.0} & 71.8\gly{+0.5} & 74.5\gly{+1.6} & 34.7\gly{+2.9} & 63.0\gly{+4.5}  \\
  \rowcolor{gray!30}
  \textbf{MCL} & \textbf{58.4}\gly{+0.9} & \textbf{84.7}\gly{+0.7} & \textbf{64.2}\gly{+1.2} & \textbf{66.5}\gly{+0.9} & \textbf{87.3}\gly{+0.3} & \textbf{72.8}\gly{+1.5} & \textbf{76.1}\gly{+3.2} & \textbf{35.7}\gly{+3.9} & \textbf{63.9}\gly{+5.4} \\ 
  \bottomrule
  \end{tabular}}
  
  \caption{Results of Mask R-CNN and Semantic FPN on COCO Keypoint and Cityscapes dataset. The results demonstrate that MCL is available for other dense prediction tasks besides detection task.}
  \label{tab:citykeypoint}
  \vspace{-5pt}
\end{table*}


==> tables/linear_eval.tex <==
\begin{table*}[h]
  \centering
  \caption{Comparison with state-of-the-art self-supervised learning methods on ImageNet-1K \textbf{linear evaluation} with the ResNet-50 backbone. Table (a) demonstrates that MCL outperforms SoCo, a state-of-the-art self-supervised pre-training for object detection. Table (b) shows that it is a trade-off between the performance of the upstream task and downstream tasks.}
  \label{tab:linear_eval}
  \vspace{-2mm}
  \begin{subtable}[t]{0.44\linewidth}
  \centering
  \vspace{0pt}
  \caption{Self-supervised learning for dense prediction.}
  \vspace{-1.2mm}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l | c | c c }
    \toprule
    Methods & Epoch & Top-1  & Top-5 \\
    \midrule
    SoCo (C4) & 100 & 59.7 & 82.8 \\
    SoCo (C4) & 400 & 62.6 & 84.6 \\
    SoCo (FPN) & 100 & 53.0 & 77.5 \\
    SoCo (FPN) & 400 & 54.2 & 79.5 \\
    SoCo* (FPN)& 400 & 53.9 & 79.2 \\
    \midrule
    MCL & 100 & 69.9 & 88.9 \\
    \rowcolor{gray!30}
    \textbf{MCL} & 400 & \textbf{71.5} & \textbf{89.9} \\
    \bottomrule
    \end{tabular}
  }
  
  \end{subtable} \hfill
  \begin{subtable}[t]{0.55\linewidth}
  \centering
  \vspace{0pt}
  \caption{Self-supervised learning for classification.}
  \vspace{-1.2mm}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l | c | c c }
    \toprule
    Methods & Epoch & Top-1  & Top-5 \\
    \midrule
    Supervised & 90 & 76.5 & - \\ 
    MoCo~\cite{he2020momentum} & 200 & 60.6 & - \\ 
    SimCLR~\cite{chen2020simple} & 1000 & 69.3 & 89.0 \\ 
    MoCo v2~\cite{chen2020improved} & 800 & 71.1 & - \\ 
    InfoMin~\cite{tian2020makes} & 800 & 73.0 & 91.1 \\ 
    BYOL~\cite{grill2020bootstrap} & 1000 & 74.3 & 91.6 \\ 
    SwAV~\cite{caron2020unsupervised} & 800 & 75.3 & - \\ 
    SimSiam~\cite{chen2021exploring} & 800 & 71.3 & - \\ 
    \bottomrule
    \end{tabular}
  }
  \end{subtable}
\end{table*}

==> tables/lvis.tex <==
\begin{table*}[t]
  
  \centering
  \resizebox{0.9\linewidth}{!}{%
  \begin{tabular}{l|llllllllllll}
  \toprule
  Methods &  AP$^\text{bb}$ & AP$_\text{50}^\text{bb}$  & AP$_\text{75}^\text{bb}$ & AP$_\text{r}^\text{bb}$  & AP$_\text{c}^\text{bb}$  & AP$_\text{f}^\text{bb}$  & AP$^\text{mk}$  & AP$_\text{50}^\text{mk}$  & AP$_\text{75}^\text{mk}$ & AP$_\text{r}^\text{mk}$ & AP$_\text{c}^\text{mk}$ & AP$_\text{f}^\text{mk}$ \\
  \midrule
  Supervised & 23.9 & 37.2 & 25.5 & 10.2 & 21.8 & 32.2 & 23.1 & 35.4 & 24.3 & 11.1 & 21.6 & 30.1 \\
  \rowcolor{gray!30}
 \textbf{MCL} & \textbf{26.2} & \textbf{40.7} & \textbf{28.4} &  \textbf{14.5} & \textbf{23.4} & \textbf{34.0} & \textbf{25.5} & \textbf{38.5} & \textbf{27.1} & \textbf{15.4} & \textbf{23.9} & \textbf{31.6}\\ 
  \bottomrule
  \end{tabular}}
  
  \caption{Transfer Learning on LVIS dataset using Mask R-CNN with R50-FPN trained for 180$k$ iterations. MCL significantly improves the performance on {\bf rare} categories by 4.3 AP$^\text{bb}$/4.3 AP$^\text{mk}$. AP$_\text{r}$, AP$_\text{c}$ and AP$_\text{f}$ are the average precision of rare, common and frequent categories, respectively.}
  \label{tab:lvis}
  \vspace{-5pt}
\end{table*}

==> tables/sup.tex <==
\begin{table*}[t]
  
  \centering
  \resizebox{0.8\linewidth}{!}{%
  \begin{tabular}{l|llllll|llllll}
  \toprule
  \multirow{2}{*}{Methods} & \multicolumn{6}{c|}{ResNet-50} & \multicolumn{6}{c}{Swin-T} \\
    & AP$^\text{bb}$ & AP$_\text{50}^\text{bb}$  & AP$_\text{75}^\text{bb}$ & AP$^\text{mk}$  & AP$_\text{50}^\text{mk}$  & AP$_\text{75}^\text{mk}$  & AP$^\text{bb}$  & AP$_\text{50}^\text{bb}$  & AP$_\text{75}^\text{bb}$ & AP$^\text{mk}$  & AP$_\text{50}^\text{mk}$  & AP$_\text{75}^\text{mk}$  \\
  \midrule
  Vanilla & 38.9 & 59.6 & 42.7 & 35.4 & 56.6 & 38.1 & 43.9 & 65.3 & 48.5 & 39.6 & 62.3 & 42.5 \\
 \rowcolor{gray!30}
 \textbf{MCL} & \textbf{42.1} & \textbf{62.6} & \textbf{45.9} & \textbf{37.8} & \textbf{59.5} & \textbf{40.6} & \textbf{44.7} & \textbf{66.0} & \textbf{49.0} & \textbf{40.3} & \textbf{62.8} & \textbf{43.4} \\ 
  \bottomrule
  \end{tabular}}
  
  \caption{Results on COCO dataset using Mask R-CNN with supervised pre-training. The results show that MCL can be extended to Swin-Transformer backbone. All the backbones are pre-trained for the same epochs. Vanilla means to pre-train model in a standard supervised manner.}
  \label{tab:sup}
  \vspace{-10pt}
\end{table*}
